A geometric method of sector decomposition

We propose a new geometric method of IR factorization in sector decomposition. The problem is converted into a set of problems in convex geometry. The latter problems are solved using algorithms in combinatorial geometry. This method provides a deterministic algorithm and never falls into an infinite loop. The number of resulting sectors depends on the algorithm of triangulation. Our test implementation shows smaller number of sectors comparing with other existing methods with iterations.

==> conclude.tex <==
\section{Conclusion}

We proposed a new method of IR factorization 
in sector decomposition
employing a geometric interpretation of the problem.
The original problem is converted into a set of problems in
convex geometry: (1) construction of intersection among dual
cones of convex polyhedral cones corresponding to each
polynomial in the original problem and (2) triangulation of
them.
They are solved by the algorithms in combinatorial geometry.
This is a deterministic method and never falls into a infinite
loop. 
The number of resulting sectors depends on the algorithm of
triangulation. 
Our test implementation of this method shows the smaller number
of sectors compared to other methods based on iterated
decomposition.


\vspace{1em}
\noindent
\textbf{Acknowledgments}

The authors wish to express their thanks to the members
of Minami-tateya group for the useful discussions.
This work is supported in part by
Ministry of Education, Science, and Culture, Japan
under Grant-in-Aid No.20340063 and No.21540286.

